Wave propagation in one-dimension: Methods and applications to complex and fractal structures

This chapter is a pedagogical review of methods and results for studying wave propagation in one-dimensional complex structures. We describe and compare the tight-binding, scattering matrix, transfer matrix and Riccati formalisms. We present examples for transport through finite-sized layered dielectric systems with periodic, quasi-periodic, fractal, disordered, and random structure, illustrating how can spatial structure affect the spectrum of modes as well as the local mode intensity.

==> ch2.tex <==
%\documentclass{psp-rv975x65}
%\usepackage{psp-rv-van}
%\makeindex
%\begin{document}

\chapter[Using Pan Stanford's Review Volume Document Style]{Using Pan Stanford's Review Volume\\ Document Style\label{ch2}}

\author[F. Author and S. Author]{First Author and Second Author\footnote{Author footnote.}}
\index[aindx]{Author, F.} % or \aindx{Author, F.}
\index[aindx]{Author, S.} % or \aindx{Author, S.}

\address{University Department, University Name, Address\\
City, State ZIP/Zone, Country\\
firstauthor\_id@domain\_name}

\begin{abstract}
The abstract should summarize the context, content and conclusions of
the paper in less than 200 words. It should not contain any references
or displayed equations. Typeset the abstract in 9 pt Times roman with
baselineskip of 11 pt, making an indentation of 1.5 pica on the left
and right margins.
\end{abstract}

\bigtoc

\tableofcontents

\body

\enlargethispage{3pt}

\section{Using Other Packages}\label{sec2.1}
The PSP class file has already loaded the packages \verb|amsfonts, amsmath,|
\verb|amssymb, epsfig, rotating,| and \verb|url| at the
startup. \verb|Check.tex| is an utility to test for all the files
required by Pan Stanford review volume project are available in
your present \LaTeX\ installation. \noindent {\bf Usage:}
\verb|latex check.tex|

Please try to limit your use of additional packages. They
frequently introduce incompatibilities. This problem is not
specific to the PSP styles, it is a general \LaTeX{} problem.
Check this manual whether the required functionality is already
provided by the PSP class file. If you do need third-party
packages, send them along with the paper. In general, you should
use standard \LaTeX{} commands as much as possible.

\section{Layout}
In order to facilitate our processing of your article, please give
easily identifiable structure to the various parts of the text by
making use of the usual \LaTeX{} commands or by your own commands
defined in the preamble, rather than by using explicit layout
commands, such as \verb|\hspace, \vspace, \large, \centering|,
etc. Also, do not redefine the page-layout parameters. For more
information on layout and font specifications please refer our
\verb|Layout Guide|.

\section{User Defined Macros}
User defined macros should be placed in the preamble of the article, and not
at any other place in the document. Such private definitions, i.e. definitions
made using the commands \verb|\newcommand, \renewcommand|, \verb|\newenvironment|
or \verb|\renewenvironment|, should be used with great care.
Sensible, restricted usage of private definitions is encouraged. Large macro
packages and Definitions that are not used in the article
should be avoided. Do not change existing environments, commands and
other standard parts of \LaTeX.

\section{Using psp-rv975x65}
You can obtain these files from our web pages at:\\
\url{http://www.panstanford.com/authors.html}.

\subsection{Input used to produce a chapter}
\begin{verbatim}
\documentclass{psp-rv975x65}
\usepackage{psp-rv-van}
\begin{document}
\chapter[Short Title]{Full Title}
\author[F. Author]{First Author}
\address{Pan Stanford Publishing...}
\begin{abstract}
The abstract should ...
\end{abstract}
\body
\section{Using Other Prepackages}
The class file has...
\begin{appendix}[Optional Appendix Title]
\section{Sample Appendix}
Text...
\end{appendix}
%\begin{thebibliography}{9}
%\bibitem{ams04} \AmS, \emph{\AmS-\LaTeX{} ...
%\end{thebibliography}
\bibliographystyle{psp-rv-van} %for BIBTeX users
\bibliography{psp-rv-sample}
\end{document}
\end{verbatim}

\section{Chapters}
Each chapter should normally be in a separate file. The chapter
title is typeset by using the \verb|\chapter[#1]{#2}| command, where
\verb|[#1]| is an optional short title to be used as a running head
if the title is too long and \verb|#2| is the full title of the
chapter. The short, edited version of the title appears in the table
of contents and running head. The chapter title should be typed in a
way such that only the initial character is in upper case and the
rest is in lower case.

\section{Sectional Units}
Sectional units are obtained in the usual way, i.e. with the \LaTeX{}
instructions \verb|\section|, \verb|\subsection|,
\verb|\subsubsection|, and \verb|\paragraph|.

\section{Section}
Text...
\subsection{Subsection}
Text...
\subsubsection{Subsubsection}
Text...
\paragraph{Paragraph}
Text...
\section*{Unnumbered Section}
Unnumbered sections can be obtained by \verb|\section*|.

\section{Lists of Items}\index{lists}
Lists are broadly classified into four major categories that can
randomly be used as desired by the author:
\begin{alphlist}[(d)]
\item Numbered list.
\item Lettered list.
\item Unnumbered list.
\item Bulleted list.
\end{alphlist}

\subsection{Numbered and lettered list}\index{lists!numbered and lettered}

\begin{enumerate}
\item The \verb|\begin{arabiclist}[]| command is used for the arabic
number list (arabic numbers appearing within parenthesis), e.g.,
(1), (2), etc.\index{lists!numbered and lettered!arabic (1, 2,
3...)}

\smallskip

\item The \verb|\begin{romanlist}[]| command is used for the roman
number list (roman numbers appearing within parenthesis), e.g., (i),
(ii), etc.\index{lists!numbered and lettered!roman (i, ii, iii...)}

\smallskip

\item The \verb|\begin{Romanlist}[]| command is used for the capital roman
\hbox{number list} (capital roman numbers appearing within
parenthesis), e.g., (I), (II), etc.\index{lists!numbered and
lettered!Roman (I, II, III...)}

\smallskip

\item The \verb|\begin{alphlist}[]| command is used for the alphabetical
list (alphabetical characters appearing within parenthesis), e.g.,
(a), (b), etc.\index{lists!numbered and lettered!alphabetical (a, b,
c...)}

\smallskip

\item The \verb|\begin{Alphlist}[]| command is used for the capital
alphabetical list (capital alphabetical characters appearing within
parenthesis), e.g., (A), (B), etc.\index{lists!numbered and lettered!Alphabetical (A, B, C...)}
\end{enumerate}
Note: For all the above mentioned lists (with the exception of
alphabetic list), it is obligatory to enter the last entry's number
in the list within the square bracket, to enable unit alignment.

\enlargethispage{\baselineskip}

Items numbered with lowercase Roman numerals:
\begin{romanlist}[(iii)]
\item item one
\item item two
    \begin{alphlist}[(a)]
    \item lists within lists can be numbered with lowercase alphabets
    \item second item.
    \end{alphlist}
\item item three.
\end{romanlist}

\subsection{Bulleted and unnumbered list}\index{lists!bulleted and unnumbered}

\begin{enumerate}
\item[] The \verb|\begin{itemlist}| command is used for the bulleted list.

\smallskip

\item[] The \verb|\begin{unnumlist}| command is used for creating the
  unnumbered list with the turnovers hangindent by 1\,pica.
\end{enumerate}

Lists may be laid out with each item marked by a dot:
\begin{itemlist}
\item item one
\item item two
\item item three.
\end{itemlist}

\subsection{Proofs}
The PSP document styles also provide a predefined proof environment for proofs.
The proof environment produces the heading
`Proof' with appropriate spacing and punctuation. A `Q.E.D.' symbol, $\square$,
can be appended at the end of a proof with the command \verb|\qed|, e.g.,

\begin{verbatim}
\begin{proof}
This is to test.
\end{proof}
\end{verbatim}

\noindent produces

\begin{proof}
This is to test.
\end{proof}

The proof environment takes an argument in curly
braces, which allows you to substitute a different name for the standard
`Proof'. If you want to display, `Proof of Lemma', then write

\begin{verbatim}
\begin{proof}[Proof of Lemma]
This is to test.
\end{proof}
\end{verbatim}

\noindent produces

\begin{proof}[Proof of Lemma]
This is to test.
\end{proof}

\section{Theorems and Definitions}\index{theorems}
The PSP document styles contain a set of pre-defined environments
for theorems, definitions, proofs, remarks etc.

\eject

The following environments are available by default with PSP document styles:

\begin{center}
{\tablefont
\begin{tabular}{ll}
\toprule Environment & Heading\\\colrule
\verb|algorithm| & Algorithm\\
\verb|answer| & Answer\\
\verb|assertion| & Assertion\\
\verb|assumption| & Assumption\\
\verb|case| & Case\\
\verb|claim| & Claim\\
\verb|comment| & Comment\\
\verb|condition| & Condition\\
\verb|conjecture| & Conjecture\\
\verb|convention| & Convention\\
\verb|corollary| & Corollary\\
\verb|criterion| & Criterion\\
\verb|definition| & Definition\\
\verb|example| & Example\\
\verb|lemma| & Lemma\\
\verb|notation| & Notation\\
\verb|note| & Note\\
\verb|observation| & Observation\\
\verb|problem| & Problem\\
\verb|proposition| & Proposition\\
\verb|question| & Question\\
\verb|remark| & Remark\\
\verb|solution| & Solution\\
\verb|step| & Step\\
\verb|summary| & Summary\\
\verb|theorem| & Theorem\\\botrule
\end{tabular}}\label{theo}
\end{center}

All theorem-like objects use individual numbering scheme by default.
To number them in a single sequence, load the class option
\verb|onethmnum| in the preamble., e.g.,
\verb|\documentclass[onethmnum]{psp-rv975x65}|.

\begin{verbatim}
\begin{theorem}
We have $\# H^2 (M \supset N) < \infty$ for an inclusion $M
\supset N$ of factors of finite index.
\end{theorem}
\end{verbatim}

\noindent produces

\begin{theorem}
We have $\# H^2 (M \supset N) < \infty$ for an inclusion $M \supset
N$ of factors of finite index.
\end{theorem}

\begin{verbatim}
\begin{theorem}[Longo, 1998]
For a given $Q$-system...
\[
N = \{x \in N; T x = \gamma (x) T, T x^* = \gamma (x^*) T\}\,,
\]
and $E_\Xi (\cdot) = T^* \gamma (\cdot) T$ gives ...
\end{theorem}
\end{verbatim}

\noindent generates

\begin{theorem}[Longo, 1998]
For a given $Q$-system...
\[
N = \{x \in N; T x = \gamma (x) T, T x^* = \gamma (x^*) T\}\,,
\]
and $E_\Xi (\cdot) = T^* \gamma (\cdot) T$ gives a conditional
expectation onto $N$.
\end{theorem}

\LaTeX{} provides \verb|\newtheorem| to create new theorem
environments. To add a new theorem-type environments to a chapter,
use

\begin{verbatim}
\newtheorem{example}{Example}[section]
\let\Examplefont\upshape
\def\Exampleheadfont{\bfseries}
\end{verbatim}

\section{Mathematical Formulas}
\paragraph{Inline:}
For in-line formulas use \verb|\( ... \) or $ ... $|. Avoid
built-up constructions, for example fractions and matrices, in
in-line formulas. Fractions in inline can be typed with a solidus e.g. \verb|x+y/z=0|.
\index{equations!inline}

\paragraph{Display:}
For numbered display formulas use the displaymath environment
\index{equations!display}
\verb|\begin{equation}...\end{equation}|.

And for unnumbered display formula use
\verb|\[ ... \]|. For numbered displayed
one line formulas always use the equation environment. Do not use
\verb|$$ ... $$|. For example, the input for:

\begin{equation}
\mu(n, t) = \frac{\sum\limits^\infty_{i=1}1(d_i < t, N(d_i) = n)}
{\int\limits^t_{\sigma=0}1(N(\sigma)=n)d\sigma}\,.
\label{eq2.1}
\end{equation}

\noindent is:

\begin{verbatim}
\begin{equation}
\mu(n,t)=\frac{\sum\limits^\infty_{i=1}1(d_i<t,N(d_i)=n)}
{\int\limits^t_{\sigma=0}1(N(\sigma)=n)d\sigma}.\label{eq2.1}
\end{equation}
\end{verbatim}

For displayed multi-line formulas use the eqnarray environment
\verb|\begin{eqnarray}...\end{eqnarray}|.

\begin{verbatim}
\begin{eqnarray}
\zeta\mapsto\hat{\zeta}&=&a\zeta+b\eta\label{eq2.2}\\
\eta\mapsto\hat{\eta}&=&c\zeta+d\eta\label{eq2.3}
\end{eqnarray}
\end{verbatim}
\noindent\begin{eqnarray}
\zeta\mapsto\hat{\zeta}&=&a\zeta+b\eta\label{eq2.2}\\
\eta\mapsto\hat{\eta}&=&c\zeta+d\eta\label{eq2.3}
\end{eqnarray}

Superscripts and subscripts that are words or abbreviations, as in
\( \pi_{\mathrm{low}} \), should be typed as roman letters; this is
done as \verb|\( \pi_{\mathrm{low}} \)| instead of \( \pi_{low} \)
done by \verb|\( \pi_{low} \)|.

For geometric functions, e.g. exp, sin, cos, tan, etc. please use the macros
\verb|\sin, \cos, \tan|. These macros gives proper spacing in mathematical formulas.

It is also possible to use the \AmS-\LaTeX{}
package,\cite{ams04} which can be obtained from the \AmS, from various \TeX{}
archives.

\section{Floats}\index{floats}
\subsection{Figures}\index{floats!figures}
A figure is obtained with the following commands

\begin{verbatim}
\begin{figure}
\psfig{file=figname.eps}
\caption{ ... caption here ... }
\label{fig2.1}
\end{figure}
\end{verbatim}
\begin{figure}
\centerline{\psfig{file=rv-fig1.eps,width=4.5cm}}
\caption{ ... caption here ... }
\label{fig2.1}
\end{figure}

\begin{figure}[t]%
\begin{center}
\subfigure[\label{fig2.2a}]{\epsfig{figure=rv-fig2a.eps,width=2.1in}}
\enskip
\subfigure[\label{fig2.2b}]{\epsfig{figure=rv-fig2b.eps,width=2.1in}}
  \caption{Here are two figures side-by-side. (a) Figure caption for figure 2a. (b) Figure caption for figure 2b.}%
  \label{fig2.2}%
\end{center}
\end{figure}
\begin{verbatim}
\begin{figure}[t]%
\begin{center}
\subfigure[\label{fig2.2a}]
          {\epsfig{figure=rv-fig2a.eps,width=2.1in}}\enskip
\subfigure[\label{fig2.2b}]
          {\epsfig{figure=rv-fig2b.eps,width=2.1in}}

\caption{Here are two figures side-by-side.
         (a) Figure caption for figure 2a.
         (b) Figure caption for figure 2b.}%\label{fig2.2}%
\end{center}
\end{figure}
\end{verbatim}

The preferred graphics are tiff and Encapsulated
PostScript, eps in short, for any type of graphic. Our
\TeX\ installation requires eps, but we can easily convert tiff to eps.
Many other formats, e.g. pict (Macintosh), wmf (Windows) and various proprietary
formats, are not suitable. Even if we can read such files, there is no guarantee
that they will look the same on our systems as on yours.

Next adjust the scaling of the figure until it's correctly positioned,
and remove the declarations of the lines and any anomalous spacing.

If instead you wish to use some other method, then it's most
important to leave the right amount of vertical space in the figure
declaration to accommodate your figure (i.e.~remove the lines and
change the space in the example).

\subsection{Tables}\index{floats!tables}
Put the tables and figures in the text with the table and figure environments,
and position them near the first reference of the table or figure in
the text. Please avoid long caption texts in figures and tables.
Do not put them at the end of the article.

\begin{table}[h]
\tbl{Sample table caption.}
{\begin{tabular}{@{}cccc@{}} \toprule
Piston mass$^{\text a}$ & Analytical frequency & TRIA6-$S_1$ model & \% Error \\
& (Rad/s) & (Rad/s) \\ \colrule
1.000 & \hphantom{0}281.0 & \hphantom{0}280.81 & 0.07 \\
0.010 & 2441.0 & 2441.00 & 0.00 \\
0.001 & 4130.0 & 4129.30 & 0.16\\ \botrule
\end{tabular}
}
\begin{tabnote}
$^{\text a}$Sample table footnote.
\end{tabnote}
\label{tbl2.1}
\end{table}

\begin{verbatim}
\begin{table}[h]
\tbl{Sample table caption.}
{\begin{tabular}{@{}cccc@{}} \toprule
Piston mass$^{\text a}$ & Analytical ...\\
& (Rad/s) & (Rad/s) \\ \colrule
1.000 & ...\\
0.001 & ...\\ \botrule
\end{tabular}}
\begin{tabnote}
$^{\text a}$Sample table footnote.
\end{tabnote}\label{tbl2.1}
\end{table}
\end{verbatim}

For most tables, the horizontal rules are obtained by:
\begin{description}\index{floats!tables!rules}
\item[toprule] one rule at the top
\item[colrule] one rule separating column heads from data cells
\item[botrule] one bottom rule
\item[Hline] one thick rule at the top and bottom of the tables with multiple column heads
\end{description}

To avoid the rules sticking out at either end
of the table add \verb|@{}| before the first and after the last descriptors, e.g.
{@{}llll@{}}. Please avoid vertical rules in tables. But if you think the vertical rule is must,
you can use the standard \LaTeX{} \verb|tabular| environment.

By using \verb|\tbl| command in table environment, long captions will
be justified to the table width while the short or single line captions
are centered. \verb|\tbl{table caption}{tabular environment}|.
If we need the fixed width for
the tables, the command is \verb|\begin{tabular*}{#1}{@{}ll@{}}|
and \verb|\end{tabular*}|. In the argument \verb|#1| the width of
the table has to be given. For example if we need the table to be
of 25pc width, then the command is
\verb|\begin{tabular*}{25pc}{@{\extracolsep{fill}}ll@{}}|.

Headings which span for more than one column should be set using
\verb|\multicolumn{#1}{#2}{#3}| where \verb|#1| is the number of
columns to be spanned, \verb|#2| is the argument for the alignment
of the column head which may be either {c} --- for center
alignment; {l} --- for left alignment; or {r} --- for right
alignment, as desired by the users. Use {c} for column heads as
this is the PSP style and \verb|#3| is the heading. A simplified
alternative version is \verb|\centre{#1}{#2}| where \verb|#1| is
the number of columns to be spanned and \verb|#2| the heading.
There should be a rule spanning the same columns below the
heading. Termed as spanner or bridge rule, it is generated using
the command \verb|\cline{n-m}| where \verb|n| is the number of the
first spanned column and \verb|m| that of the last spanned column.
\verb|\cline| should not be part of a row but follow immediately
after a \verb|\\|.

If a table contains note(s), as a
universal thumb-rule they should appear beneath the table set to its
width and seldom at the foot of the page. For the footnotes in the
table environment the command is
\verb|{\begin{tabnote}<text>| \verb|\end{tabnote}}|. Appropriate symbols
should be included in the body of the table matching their
corresponding symbols in the footnotes where the footnotes are to be
placed immediately after the \verb|{\begin{tabnote}| command and
terminated before \verb|\end{tabnote}}\end{table}| command.

\def\p{\phantom{$-$}}
\def\pc{\phantom{,}}
\def\p0{\phantom{0}}
\begin{sidewaystable*}
\tbl{Positive values of $X_0$ by eliminating $Q_0$ from Eqs.~(15)
and (16) for different values of the parameters $f_0$, $\lambda_0$
and $\alpha_0$ in various dimension.}
{\begin{tabular}{@{}ccccccccccc@{}}
\toprule\\[-6pt]
$f_0$ &$\lambda_0$ &$\alpha_0$
&\multicolumn{8}{c}{Positive roots ($X_0$)}\\[3pt]
\hline\\[-6pt]
&& &4D &5D &6D &7D &8D &10D &12D &16D\\[3.5pt]
\hline\\[-6pt]
\phantom{1}$-0.033$ &0.034 &\phantom{0}0.1\phantom{.01}
&6.75507,\p0 &4.32936,\p0 &3.15991,\p0 &2.44524,\p0
&1.92883,\p0 &0.669541, &--- &---\\[3.5pt]
&&&1.14476\pc\p0 &1.16321\pc\p0 &1.1879\pc\phantom{00}
&1.22434\pc\p0 &1.29065\pc\p0
&0.415056\pc\\[3.5pt]
\phantom{1}$-0.1$\phantom{33} &0.333 &\phantom{0}0.2\phantom{.01}
&3.15662,\p0 &1.72737,\p0 &--- &--- &--- &--- &--- &---\\[3.5pt]
&&&1.24003\pc\p0 &1.48602\pc\p0\\[3.5pt]
\phantom{1}$-0.301$ &0.302 &0.001
&2.07773,\p0 &--- &--- &--- &--- &--- &--- &---\\[3.5pt]
&&&1.65625\pc\p0\\[3.5pt]
\phantom{1}$-0.5$\phantom{01} &0.51\phantom{2} &\phantom{0}0.001
&--- &--- &--- &--- &--- &--- &--- &---\\[3.5pt]
$\phantom{1-}$0.1\phantom{01} &0.1\phantom{02}
&\phantom{0}2\phantom{.001} &1.667,\phantom{000} &1.1946\phantom{00,}
&--- &--- &--- &--- &--- &---\\[3.5pt]
&&&0.806578\pc &0.858211\pc\\[3.5pt]
$\phantom{1-}$0.1\phantom{01} &0.1\phantom{33} &10\phantom{.001}
&0.463679\pc &0.465426\pc &0.466489\pc &0.466499\pc
&0.464947\pc &0.45438\pc\p0 &0.429651\pc &0.35278\pc\\[3.5pt]
$\phantom{1-}$0.1\phantom{01} &1\phantom{.333}
&\phantom{0}0.2\phantom{01}
&--- &--- &--- &--- &--- &--- &--- &---\\[3.5pt]
$\phantom{-0}$1\phantom{.033} &0.001 &\phantom{0}2\phantom{.001}
&0.996033, &0.968869, &0.91379,\p0 &0.848544,&0.783787, &0.669541,
&0.577489, &---\\[3.5pt]
&&&0.414324\pc &0.41436\pc\p0 &0.414412\pc &0.414489\pc &0.414605\pc
&0.415056\pc &0.416214\pc\\[3.5pt]
\phantom{10}\phantom{.033} &0.001 &\phantom{0}0.2\phantom{01}
&0.316014, &0.309739, &--- &--- &--- &--- &--- &---\\[3.5pt]
&&&0.275327\pc &0.275856\pc\\[3.5pt]
\phantom{10}\phantom{.033} &0.1\phantom{33}
&\phantom{0}5\phantom{.001}
&0.089435\pc &0.089441\pc &0.089435\pc &0.089409\pc &0.08935\pc\p0
&0.089061\pc &0.088347\pc &0.084352\pc\\[3.5pt]
\phantom{10}\phantom{.033} &1\phantom{.333} &\phantom{0}3\phantom{.001}
&0.128192\pc &0.128966\pc &0.19718,\p0 &0.169063, &0.142103,
&--- &--- &---\\[3.5pt]
&&&& &0.41436\pc\p0 &0.414412\pc &0.414489\pc\\[3pt]
\Hline
\end{tabular}}\label{tbl2}
\end{sidewaystable*}

\begin{sidewaysfigure}
\begin{center}
\psfig{file=rv-fig3.eps,width=6.6in}
\end{center}
\caption{Very large figures and tables should be placed on a page
by themselves..}
\label{fig3}
\end{sidewaysfigure}

The tables are designed to have a uniform style throughout the whole
book. We prefer the border lines to be of the style as shown in our
sample Tables. For the inner lines of the table, it looks better if
they are kept to a minimum.

Landscape tables and figures can be typeset with following environments:
\begin{itemize}\index{floats!tables!landscape}
\item \verb|sidewaystable| and
\item \verb|sidewaysfigure|.
\end{itemize}

\noindent {\bf Example:}

\begin{verbatim}
\begin{sidewaystable*}
\tbl{Positive values of ...}
{\begin{tabular}{@{}ccccccccccc@{}}
\toprule\\
$f_0$ &$\lambda_0$ &$\alpha_0$...
...\\ \botrule
\end{tabular}}
\label{tbl2}
\end{sidewaystable*}

\begin{sidewaysfigure}
\begin{center}
\psfig{file=rv-fig3.eps,width=6.6in}
\end{center}
\caption{The bifurcating response ...}
\label{fig3}
\end{sidewaysfigure}
\end{verbatim}

\section{Cross-references}
Use \verb|\label| and \verb|\ref| for cross-references to
equations, figures, tables, sections, subsections, etc., instead
of plain numbers. Every numbered part to which one wants to refer,
should be labelled with the instruction \verb|\label|.
For example:
\begin{verbatim}
\begin{equation}
\mu(n, t) = \frac{\sum\limits^\infty_{i=1}1
(d_i < t, N(d_i) = n)}
{\int\limits^t_{\sigma=0}1
(N(\sigma)=n)d\sigma}\,.\label{eq2.1}
\end{equation}
\end{verbatim}
With the instruction \verb|\ref| one can refer to a numbered part
that has been labelled:
\begin{verbatim}
..., see also Eq. (\ref{eq2.1})
\end{verbatim}
\begin{itemize}
\item The \verb|\label| instruction should be typed
immediately after (or one line below), e.g.,
\verb|\caption{ ... caption ... }\label{fig2.1.1}|. Labels should not be typed inside the argument of
a number-generating instruction such as \verb|\section| or \verb|\caption|,
\item For chapters, labels should be placed inside \verb|\chapter|, e.g.,\\
    \verb|\chapter{Chapter Title\label{ch2}}|.
\item labels should not be repeated.
\end{itemize}

\begin{center}{\tablefont
Some useful shortcut commands.\\
\begin{tabular}{lll}
\toprule
Shortcut & Equivalent & Output \\
command & \TeX\ command\\\colrule
\multicolumn{3}{@{}l}{In the middle of a sentence:}\\
\verb|\eref{eq2.1}|  & Eq.~(\verb|\ref{eq2.1}|) & \eref{eq2.1}\\
\verb|\sref{sec2.1}| & Sec.~\verb|\ref{sec2.1}| & \sref{sec2.1}\\
\verb|\cref{ch2}|  & Chap.~\verb|\ref{ch2}| & \cref{ch2}\\
\verb|\fref{fig2.1}| & Fig.~\verb|\ref{fig2.1}|  & \fref{fig2.1}\\
\verb|\tref{tbl2.1}| & Table~\verb|\ref{tbl2.1}|  & \tref{tbl2.1}\\[3pt]
\multicolumn{2}{@{}l}{At the starting of a sentence:}\\
\verb|\Eref{eq2.1}|  & Equation (\verb|\ref{eq2.1}|) & \Eref{eq2.1}\\
\verb|\Sref{sec2.1}| & Section~\verb|\ref{sec2.1}| & \Sref{sec2.1}\\
\verb|\Cref{ch2}|  & Chapter~\verb|\ref{ch2}| & \Cref{ch2}\\
\verb|\Fref{fig2.1}| & Figure~\verb|\ref{fig2.1}| & \Fref{fig2.1}\\
\verb|\Tref{tbl2.1}| & Table~\verb|\ref{tbl2.1}| & \Tref{tbl2.1}\\\botrule
\end{tabular}}
\end{center}

\section{Citations}\label{cit}\index{citation}

Pan Stanford's preferred style for Review Volume is the Vancouver (numbered) system,
unless if the text is not very heavily referenced in which case the
Harvard (author-date) system may be used.

\begin{center}
\tablefont
\begin{tabular}{@{}ll@{}}\toprule
System & Package\\\colrule
 Vancouver (numbered)\\
 \quad$\bullet$ Bracketed [1] & \verb|\usepackage[square]{psp-rv-van}|\\
 \quad$\bullet$ Superscript$^1$ & \verb|\usepackage{psp-rv-van}| (Default style)\\[3pt]
 Harvard (author-date) & \verb|\usepackage{psp-rv-har}|\\\botrule
\end{tabular}
\end{center}

Citations in the text use the labels defined in the bibitem declaration,
for example, the first paper by Jarlskog\cite{jarl88} is cited using the
command \verb|\cite{jarl88}|. The bibitem labels should not be repeated.
For multiple citations do not use \verb|\cite{1}\cite{2}|, but use
\verb|\cite{1,2}| instead.
When superscripted citations are used, there should not be a space
before \verb|\cite{key}|, e.g.,

\

citation:
\verb|see\cite{zipf}|\hskip-60pt\lower8pt\hbox{$\uparrow$}\hskip-4pt\lower16pt\hbox{no
character space here}

\

\noindent Reference: \verb|\bibitem{zipf} E. Zipf, {\it Bull. Am. Phys.Soc.} {\bf 15}, 418 (1970).|

\subsubsection*{Output:}

citation: ...text.$^1$

...

\noindent{\bf Reference}

\noindent {\bibfont 1.  E. C. Zipf, {\it Bull. Am. Phys. Soc.} {\bf 15}, 418
(1970).}

\subsection{Vancouver Style}\index{citation!numbered}

Reference citations in the text are to be numbered consecutively in
Arabic numerals, in the order of first appearance. The numbered citations
can appear in two ways:

\begin{romanlist}[(ii)]
\item bracketed
\item superscript (default style)
\end{romanlist}

\subsubsection{Bracketed}\index{citation!numbered!bracketed}
References cited in the text are within square brackets, e.g.,

\begin{arabiclist}[(2)]
\item \verb|``One can deduce from Ref.~\cite{benh93} that...''|\\
            ``One can deduce from Ref.~[3] that...''
\smallskip
\item \verb|``See Refs.~\cite{ams04,bake72,benh93,brow88} and|\\
      \verb|\cite{davi93} for more details.''|\\
      ``See Refs.~[1--3, 5] and [7] for more details.''
\end{arabiclist}

\subsubsection{Superscript}\index{citation!numbered!superscript}

References cited in the text appear as superscripts, e.g.,

\begin{arabiclist}[(2)]
\item \verb|``...in the statement.\cite{ams04}''|\\
            ``...in the statement.$^1$''
\smallskip
\item \verb|``...have proven\cite{bake72} that this equation...''|\\
            ``...have proven$^2$ that this equation...''
\end{arabiclist}

When the reference forms part of the sentence, it should appear with
``Reference'' or ``Ref.'', e.g.,

\begin{arabiclist}[(2)]
\item \verb|``One can deduce from Ref.~\refcite{benh93} that...''|\\
      ``One can deduce from Ref.~3 that...''
\smallskip
\item \verb|``See Refs.~\refcite{ams04}--\refcite{benh93},|
      \verb|\refcite{brow88} and \refcite{davi93} for more details.''|\\
     ``See Refs.~1--3, 5 and 7 for more details.''
\end{arabiclist}

\subsection{Harvard Style}\index{citation!author-date}
Citations in the
text use the labels defined in the \verb|bibitem| declaration, for example,
the first paper by [Jarlskog (1988)] is cited using the command
\verb|\cite{jarl88}|. See Sec.~\ref{secbib} for more details on coding references in Vancouver and Harvard style.

\section{Footnote}
Footnotes are denoted by a Roman letter superscript in the text. Footnotes can be used as

\begin{verbatim}
... total.\footnote{Sample footnote text.}
\end{verbatim}

\noindent {\bf Output:}

\noindent ... in total.\footnote{Sample footnote text.}

\section{Acknowledgments}
Acknowledgments to funding bodies etc. may be placed in a separate
section at the end of the text, before the Appendices. This should not
be numbered so use \verb|\section*{Acknowledgements}|.

\section{Appendix}\index{appendix}
Appendices should be used only when absolutely necessary. They
should come before the References.

\begin{verbatim}
\begin{appendix}[Optional Appendix Title]
\section{Sample Appendix}
Text...
\subsection{Appendix subsection}
Text...
\begin{equation}
\mu(n, t) = ...\label{appen1}
\end{equation}
\section{Sample Head}
Text...
\end{appendix}
\end{verbatim}

\section{Bibliography}\label{secbib}\index{bibliography}
Use \verb|\bibitem| to produce the bibliography.
The bibitem labels should not be repeated.

\subsection{\btex\ users}

\btex\index{BIBTeX} users should use our bibliography style file
\verb|psp-rv-van.bst| or \verb|psp-rv-har.bst|.
\Cref{ch3} of this document has more on \btex.

\subsection{Non-\btex\ users}
For Vancouver (numbered) style users, references are to be listed in the order cited in the text. Use the
style shown in the following examples.

\begin{verbatim}
\begin{thebibliography}{9}
\bibitem{ams04}
\AmS, \emph{\AmS-\LaTeX{} Version 2 User's Guide}.
   (American Mathematical Society, Providence, 2004).
   \url{http://www.ams.org/tex/amslatex.html}.

\bibitem{jarl88}
C.~Jarlskog, \emph{CP Violation}. (World Scientific,
   Singapore, 1988).

\bibitem{best03}
B.~W. Bestbury, {$R$}-matrices and the magic square,
   \emph{J. Phys. A}. {\bf 36} (7), 1947--1959, (2003).

\bibitem{pier02}
P.~X. Deligne and B.~H. Gross, On the exceptional series,
  and its descendants, \emph{C. R. Math. Acad. Sci. Paris}.
  {\bf 335} (11), 877--881, (2002).

\end{thebibliography}
\end{verbatim}

For Harvard (author-date) style users, the references are to be listed in
alphabetical order according to the surname of the first author.
Use the style shown in the following examples.

\begin{verbatim}
\begin{thebibliography}{9}

\bibitem[{Baker and Carter(1972)}]{bake72}
Baker, D.~W. and Carter, N.~L. (1972). {\it Seismic Velocity
   Anisotropy Calculated for Ultramafic Minerals and
   Aggregates}, \emph{Geophys. Mono.}, Vol.~16 (Am. Geophys.
   Union), pp. 157--166.

\bibitem[{Benhamou and Colmerauer(1993)}]{benh93}
Benhamou, F. and Colmerauer, A. (eds.) (1993). {\it Constraint
   Logic Programming, Selected Research} (MIT Press).

\bibitem[{Bestbury(2003)}]{best03}
Bestbury, B.~W. (2003). {$R$}-matrices and the magic
   square, \emph{J. Phys. A} \textbf{36}, 7, pp. 1947--1959.

\bibitem[{Brown(1988)}]{brow88}
Brown, M.~E. (1988). {\it An Interactive Environment for Literate
   Programming}, Ph.D. thesis, Texas A\&M University, TX, USA.
\bibitem[{Churchill and Brown(1990)}]{chur90}
Churchill, R.~V. and Brown, J.~W. (1990). \emph{Complex
   Variables and Applications}, 5th edn. (McGraw-Hill).

\end{thebibliography}
\end{verbatim}

\begin{appendix}[Appendix Title]
\section{Appendices}\index{appendix}
Appendices should be used only when absolutely necessary. They
should come before the References. If there is more than one
appendix, number them alphabetically.
Sectional units are obtained in the usual way, i.e. with the
\LaTeX{} instructions \verb|\section|, \verb|\subsection|.

\begin{table}[b]
\tbl{Commonly used macros.}{
\begin{tabular}{@{}ll@{}}
\toprule
Macro name&Purpose\\
\colrule
{\tt$\backslash$chapter[\#1]}\{{\tt\#2}\} & Chapter title\\
{\tt$\backslash$author[\#1]}\{{\tt\#2}\} & Author Name(S)\\
{\tt$\backslash$address}\{{\tt\#1}\} & Address\\
{\tt$\backslash$begin}\{{\tt{abstract}}\} & Start Abstract\\
{\tt$\backslash$end}\{{\tt{abstract}}\} & End Abstract\\
{\tt$\backslash$bigtoc} & For longer TOCs (e.g. 1.99. Section Title)\\
{\tt$\backslash$smalltoc} & For smaller TOCs (e.g. 1.9. Section Title)\\
{\tt$\backslash$tableofcontents} & Table of Contents\\
{\tt$\backslash$body} & Start Body Text\\
{\tt$\backslash$section}\{{\tt\#1}\} & Section heading\\
{\tt$\backslash$subsection}\{{\tt\#1}\} & Subsection heading\\
{\tt$\backslash$subsubsection}\{{\tt\#1}\} & Subsubsection heading\\
{\tt$\backslash$section*}\{{\tt\#1}\} & Unnumbered Section head\\
{\tt$\backslash$begin}\{{\tt{itemlist}}\} & Start bulleted lists\\
{\tt$\backslash$end}\{{\tt{itemlist}}\} & End bulleted lists\\
{\tt$\backslash$begin}\{{\tt{arabiclist}}\} & Start arabic lists (1, 2, 3...)\\
{\tt$\backslash$end}\{{\tt{arabiclist}}\} & End arabic lists\\
{\tt$\backslash$begin}\{{\tt{romanlist}}\} & Start roman lists (i, ii, iii...)\\
{\tt$\backslash$end}\{{\tt{romanlist}}\} & End roman lists\\
{\tt$\backslash$begin}\{{\tt{Romanlist}}\} & Start roman lists (I, II, III...)\\
{\tt$\backslash$end}\{{\tt{Romanlist}}\} & End roman lists\\
{\tt$\backslash$begin}\{{\tt{alphlist}}\} & Start alpha lists (a, b, c...)\\
{\tt$\backslash$end}\{{\tt{alphlist}}\} & End alpha lists\\
{\tt$\backslash$begin}\{{\tt{Alphlist}}\} & Start alpha lists (A, B, C...)\\
{\tt$\backslash$end}\{{\tt{Alphlist}}\} & End alpha lists\\
{\tt$\backslash$begin}\{{\tt{proof}}\} & Start of Proof\\
{\tt$\backslash$end}\{{\tt{proof}}\} & End of Proof\\
{\tt$\backslash$begin}\{{\tt{theorem}}\} & Start of Theorem\\
{\tt$\backslash$end}\{{\tt{theorem}}\} & End of Theorem (see Page \pageref{theo} for detailed list)\\
{\tt$\backslash$begin}\{{\tt{appendix}}\}[{\tt\#1}] & Start Appendix\\
{\tt$\backslash$end}\{{\tt{appendix}}\} & End Appendix\\
{\tt$\backslash$begin}\{{\tt{thebibliography}}\}\{{\tt\#1}\} & Start of reference list\\
{\tt$\backslash$end}\{{\tt{thebibliography}}\} & End of reference list\\
{\tt$\backslash$bibitem}[\{{\tt\#1}\}]\{{\tt\#2}\}& reference item in author-date style\\
{\tt$\backslash$bibitem}\{{\tt\#1}\} & reference item in numbered style\\
{\tt$\backslash$bibliographystyle}\{{\tt\#1}\} & To include \btex{} style file\\
{\tt$\backslash$bibliography}\{{\tt\#1}\} & To include \btex{} database\\ \botrule
\end{tabular}}
\end{table}

\begin{table}[t]
\tbl{Macros available for Tables/Figures.}{
\begin{tabular}{@{}ll@{}}
\toprule
Environment name&Purpose\\
\colrule
{\tt figure} & figures\\
{\tt sidewaysfigure} & landscape figures\\
{\tt table} & tables\\
{\tt sidewaystable} & landscape tables\\
{\tt$\backslash$tbl}\{{\tt\#1}\}\{{\tt\#2}\} & \#1 - table caption;\\
& \#2 - tabular environment\\[3pt]
\multicolumn{2}{@{}l}{Horizantal Rules for tables}\\
{\tt$\backslash$toprule} & one rule at the top\\
{\tt$\backslash$colrule} & one rule separating column heads from\\ & data cells\\
{\tt$\backslash$botrule} & one bottom rule\\
{\tt$\backslash$Hline} & one thick rule at the top and bottom of\\ & the tables with multiple column heads\\
\botrule
\end{tabular}}
\end{table}

\subsection{Appendix sectional units}
Number displayed equations
occurring in the Appendix in this way, e.g.~(\ref{appeq1}), (A.2),
etc.

\begin{equation}
\mu(n, t) = \frac{\sum\limits^\infty_{i=1}1
(d_i < t, N(d_i) = n)}
{\int\limits^t_{\sigma=0}1(N(\sigma)=n)d\sigma}\,.
\label{appeq1}
\end{equation}

\end{appendix}

\bibliographystyle{psp-rv-van}
\bibliography{psp-rv-sample1}

%\end{document}


==> check.tex <==
%% Usage: Latex check.tex
%%
%% Utility to test if all the files required for wspc review volume project
%% are available in your present LaTeX path.
%% - psp-rv975x65.cls
%% - epsfsafe.tex
%% - rotating.sty
%% - url.sty
%% - makeidx.sty
%% - chapterbib.sty
%% - overcite.sty
%% - psp-index.sty

\newif\onerror

\typeout{*}
\typeout{1. Searching for LaTeX2e ... }
\ifx\documentclass\undefined
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* The PSP Review Volume class can only be used with LaTeX2e}
 \typeout{*}
 \typeout{* Stopping...}
 \expandafter\stop
\else
 \typeout{   ... ok}
\fi

\def\next#1/#2/#3\next{#1#2}
\typeout{ }
\typeout{2.  Searching for LaTeX2e version ... }
\ifnum\expandafter\next\fmtversion\next<199612 \relax
 \typeout{*}
 \typeout{* Fatal error occurred:}
 \typeout{*}
 \typeout{* Your LaTeX version is quite outdated, \fmtversion.}
 \typeout{* The PSP Review Volume class can only be used with}
 \typeout{* a recent version of LaTeX2e, please upgrade your installation!}
 \typeout{*}
 \expandafter\stop
\else
 \ifnum\expandafter\next\fmtversion\next<199806 \relax
   \typeout{* Warning: }
   \typeout{*}
   \typeout{* Your LaTeX version is outdated, \fmtversion.}
   \typeout{* We believe that it will probably work, but if you encounter}
   \typeout{* problems you will need upgrade your installation.}
   \typeout{*}
   \typein{* Type <return> to continue ...}
   \errortrue
 \else
   \typeout{   ... ok}
 \fi
\fi

\typeout{ }
\typeout{3. Searching for psp-rv975x65.cls ... }
\IfFileExists{psp-rv975x65.cls}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{* ... psp-rv975x65.cls, file not found! }
     \typeout{*}
     \typeout{* Fatal error occurred:}
     \typeout{*}
     \typeout{* The psp-rv975x65 class file which is part of the PSP Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }
\typeout{4. Searching for epsfsafe.tex ... }
\IfFileExists{epsfsafe.tex}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... epsfsafe.tex, file not found! }
     \typeout{*}
     \typeout{*}
     \typeout{* The epsfsafe.tex file which is part of the PSP Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* Stopping...}
     \typeout{*}
     \stop
}

\typeout{ }
\typeout{5. Searching for rotating.sty ... }
\IfFileExists{rotating.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... rotating.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The rotating package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use}
     \typeout{* sidewaysfigure and sidewaystable environments.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "rotating".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{6. Searching for url.sty ... }
\IfFileExists{url.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... url.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The url package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to use the \string\url}
     \typeout{* command. Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "url".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{7. Searching for makeidx.sty ... }
\IfFileExists{makeidx.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... makeidx.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The makeidx package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to generate index.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "makeidx".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{8. Searching for chapterbib.sty ... }
\IfFileExists{chapterbib.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... chapterbib.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The chapterbib package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to include separate bibliography for each chapter.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "chapterbib".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{9. Searching for overcite.sty ... }
\IfFileExists{overcite.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... overcite.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The overcite package, which should be part of a good LaTeX}
     \typeout{* distribution, can not be found.}
     \typeout{*}
     \typeout{* Without this package you will not be able to generate citations in superscript.}
     \typeout{* Try to download this package from a CTAN host.}
     \typeout{* Go to http://www.ctan.org/search.html and search for "overcite".}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{10. Searching for psp-rv-har.bst ... }
\IfFileExists{psp-rv-har.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... psp-rv-har.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The psp-rv-har bibliography style file which is part of the PSP Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the psp-rv975x65 class without this package but }
     \typeout{* you can not use BiBTeX features.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{11. Searching for psp-rv-van.bst ... }
\IfFileExists{psp-rv-van.bst}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... psp-rv-van.bst, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The psp-rv-van bibliography style file which is part of the PSP Review Volume distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the psp-rv975x65 class without this package but }
     \typeout{* you can not use BiBTeX features.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{12. Searching for psp-index.sty ... }
\IfFileExists{psp-index.sty}
    {
     \typeout{  ... ok}
    }
    {
     \typeout{  ... psp-index.sty, file not found! }
     \typeout{ }
     \typeout{* Warning:}
     \typeout{*}
     \typeout{* The psp-index package which is part of the PSP RV distribution}
     \typeout{* must be installed in a directory which is searched by LaTeX.}
     \typeout{*}
     \typeout{* You can use the psp-rv975x65 class without this package but }
     \typeout{* you can not use multiple indexes.}
     \typeout{*}
     \typeout{*}
     \typein{* Type <return> to continue ...}
     \errortrue
    }

\typeout{ }
\typeout{* Finished Testing *}
\typeout{ }
\onerror
\typeout{* Some of the file(s) required by PSP was not found.}
\typeout{* Please review the above comments carefully and update your system.}
\typeout{*}
\typeout{* PSP files can be downloaded from:}
\typeout{* http://www.panstanford.com/authors.html}
\typeout{*}
\typeout{* Other TeX packages can be downloaded from:}
\typeout{* http://www.ctan.org/search.html}
\typeout{*}
\typeout{* For technical support, please email Rajesh <rajesh@wspc.com.sg>.}
\typeout{*}
\typeout{******************************************************************}
\typein{* Type <return> to continue ...} \else
\typeout{******************************************************************}
\typeout{*}
\typeout{* All the files and packages required by PSP was found,}
\typeout{* you may now proceed LaTeXing your files.}
\typeout{*}
\typeout{* Latest TeX packages can be downloaded from:}
\typeout{* http://www.ctan.org/search.html}
\typeout{*}
\typeout{* For technical support, please email Rajesh <rajesh@wspc.com.sg>.}
\typeout{*}
\typeout{******************************************************************}
\fi
\stop
\endinput


==> epsfsafe.tex <==
%   EPSF.TEX macro file (modified for EPSF images with TIFF preview)
%
%   Written by Tomas Rokicki of Radical Eye Software, 29 Mar 1989.
%   Revised by Don Knuth, 3 Jan 1990.
%   Revised by Tomas Rokicki to accept bounding boxes with no
%	space after the colon, 18 Jul 1990.
%-%   Modified to deal with %%BoundingBox: (at end) as well as TIFF 
%-%	preview in EPSF format files, 1993 Jan 23 (see %-% comments).
%
%   TeX macros to include an Encapsulated PostScript graphic.
%   Works by finding the bounding box comment,
%   calculating the correct scale values, and inserting a vbox
%   of the appropriate size at the current position in the TeX document.
%
%   To use with the center environment of LaTeX, preface the \epsffile
%   call with a \leavevmode.  (LaTeX should probably supply this itself
%   for the center environment.)
%
%   To use, simply say
%   \input epsfsafe	  % somewhere early on in your TeX file
%   \epsfbox{filename.ps} % where you want to insert a vbox for a figure
%
%   Alternatively, you can type
%
%   \epsfbox[0 0 30 50]{filename.ps} % to supply your own BB
%
%   which will not read in the file, and will instead use the bounding
%   box you specify.
%
%   The effect will be to typeset the figure as a TeX box, at the
%   point of your \epsfbox command. By default, the graphic will have its
%   `natural' width (namely the width of its bounding box, as described
%   in filename.ps). The TeX box will have depth zero.
%
%   You can enlarge or reduce the figure by saying
%     \epsfxsize=<dimen> \epsfbox{filename.ps}
%   (or
%     \epsfysize=<dimen> \epsfbox{filename.ps})
%   instead. Then the width of the TeX box will be \epsfxsize and its
%   height will be scaled proportionately (or the height will be
%   \epsfysize and its width will be scaled proportiontally).  The
%   width (and height) is restored to zero after each use.
%
%   A more general facility for sizing is available by defining the
%   \epsfsize macro.  Normally you can redefine this macro
%   to do almost anything.  The first parameter is the natural x size of
%   the PostScript graphic, the second parameter is the natural y size
%   of the PostScript graphic.  It must return the xsize to use, or 0 if
%   natural scaling is to be used.  Common uses include:
%
%      \epsfxsize  % just leave the old value alone
%      0pt	   % use the natural sizes
%      #1	   % use the natural sizes
%      \hsize	   % scale to full width
%      0.5#1	   % scale to 50% of natural size
%      \ifnum#1>\hsize\hsize\else#1\fi	% smaller of natural, hsize
%
%   If you want TeX to report the size of the figure (as a message
%   on your terminal when it processes each figure), say `\epsfverbosetrue'.
%
\chardef\quoteleftcode=\catcode96	% remember catcode of `
\catcode96=12				% make sure ` is "ordinary"

\newread\epsffilein    % file to \read
\newif\ifepsffileok    % continue looking for the bounding box?
\newif\ifepsfbbfound   % success?
\newif\ifepsfverbose   % report what you're making?
\newdimen\epsfxsize    % horizontal size after scaling
\newdimen\epsfysize    % vertical size after scaling
\newdimen\epsftsize    % horizontal size before scaling
\newdimen\epsfrsize    % vertical size before scaling
\newdimen\epsftmp      % register for arithmetic manipulation
\newdimen\pspoints     % conversion factor
%
\pspoints=1bp	       % Adobe points are `big'
\epsfxsize=0pt	       % Default value, means `use natural size'
\epsfysize=0pt	       % ditto
%
\def\epsfbox#1{\global\def\epsfllx{72}\global\def\epsflly{72}%
   \global\def\epsfurx{540}\global\def\epsfury{720}%
   \def\lbracket{[}\def\testit{#1}\ifx\testit\lbracket
   \let\next=\epsfgetlitbb\else\let\next=\epsfnormal\fi\next{#1}}%
%
\def\epsfgetlitbb#1#2 #3 #4 #5]#6{\epsfgrab #2 #3 #4 #5 .\\%
   \epsfsetgraph{#6}}%
%
\def\epsfnormal#1{\epsfgetbb{#1}\epsfsetgraph{#1}}%
%
\def\epsfgetbb#1{%
%
%   The first thing we need to do is to open the
%   PostScript file, if possible.
%
\openin\epsffilein=#1
\ifeof\epsffilein\errmessage{I couldn't open #1, will ignore it}\else
%
%   Okay, we got it. Now we'll scan lines until we find one that doesn't
%   start with %. We're looking for the bounding box comment.
%
   {\epsffileoktrue \chardef\other=12
    \def\do##1{\catcode`##1=\other}\dospecials \catcode`\ =10
%-% Neuter some more nasty characters
    \catcode`\^^L=9 \catcode`\^^?=9
    \loop
       \read\epsffilein to \epsffileline
       \ifeof\epsffilein\epsffileokfalse\else
%
%   We check to see if the first character is a % sign;
%   if not, we stop reading (unless the line was entirely blank);
%   if so, we look further and stop only if the line begins with
%   `%%BoundingBox:'.
%
	  \expandafter\epsfaux\epsffileline:. \\%
       \fi
   \ifepsffileok\repeat
   \ifepsfbbfound\else
    \ifepsfverbose\message{No bounding box comment in #1; using defaults}\fi\fi
   }\closein\epsffilein\fi}%
%
%   Now we have to calculate the scale and offset values to use.
%   First we compute the natural sizes.
%
\def\epsfclipstring{}% do we clip or not?  If so,
\def\epsfclipon{\def\epsfclipstring{ clip}}%
\def\epsfclipoff{\def\epsfclipstring{}}%
%
\def\epsfsetgraph#1{%
   \epsfrsize=\epsfury\pspoints
   \advance\epsfrsize by-\epsflly\pspoints
   \epsftsize=\epsfurx\pspoints
   \advance\epsftsize by-\epsfllx\pspoints
%
%   If `epsfxsize' is 0, we default to the natural size of the picture.
%   Otherwise we scale the graph to be \epsfxsize wide.
%
   \epsfxsize\epsfsize\epsftsize\epsfrsize
   \ifnum\epsfxsize=0 \ifnum\epsfysize=0
      \epsfxsize=\epsftsize \epsfysize=\epsfrsize
      \epsfrsize=0pt
%
%   We have a sticky problem here:  TeX doesn't do floating point arithmetic!
%   Our goal is to compute y = rx/t. The following loop does this reasonably
%   fast, with an error of at most about 16 sp (about 1/4000 pt).
%
     \else\epsftmp=\epsftsize \divide\epsftmp\epsfrsize
       \epsfxsize=\epsfysize \multiply\epsfxsize\epsftmp
       \multiply\epsftmp\epsfrsize \advance\epsftsize-\epsftmp
       \epsftmp=\epsfysize
       \loop \advance\epsftsize\epsftsize \divide\epsftmp 2
       \ifnum\epsftmp>0
          \ifnum\epsftsize<\epsfrsize\else
	     \advance\epsftsize-\epsfrsize \advance\epsfxsize\epsftmp \fi
       \repeat
       \epsfrsize=0pt
     \fi
   \else \ifnum\epsfysize=0
     \epsftmp=\epsfrsize \divide\epsftmp\epsftsize
     \epsfysize=\epsfxsize \multiply\epsfysize\epsftmp
     \multiply\epsftmp\epsftsize \advance\epsfrsize-\epsftmp
     \epsftmp=\epsfxsize
     \loop \advance\epsfrsize\epsfrsize \divide\epsftmp 2
     \ifnum\epsftmp>0
	\ifnum\epsfrsize<\epsftsize\else
	   \advance\epsfrsize-\epsftsize \advance\epsfysize\epsftmp \fi
     \repeat
     \epsfrsize=0pt
    \else
     \epsfrsize=\epsfysize
    \fi
   \fi
%
%  Finally, we make the vbox and stick in a \special that dvips can parse.
%
   \ifepsfverbose\message{#1: width=\the\epsfxsize, height=\the\epsfysize}\fi
   \epsftmp=10\epsfxsize \divide\epsftmp\pspoints
   \vbox to\epsfysize{\vfil\hbox to\epsfxsize{%
      \ifnum\epsfrsize=0\relax
        \special{PSfile=#1 llx=\epsfllx\space lly=\epsflly\space
            urx=\epsfurx\space ury=\epsfury\space rwi=\number\epsftmp
            \epsfclipstring}%
      \else
        \epsfrsize=10\epsfysize \divide\epsfrsize\pspoints
        \special{PSfile=#1 llx=\epsfllx\space lly=\epsflly\space
            urx=\epsfurx\space ury=\epsfury\space rwi=\number\epsftmp\space
            rhi=\number\epsfrsize \epsfclipstring}%
      \fi
      \hfil}}%
\global\epsfxsize=0pt\global\epsfysize=0pt}%
%
%   We still need to define the tricky \epsfaux macro. This requires
%   a couple of magic constants for comparison purposes.
%
{\catcode`\%=12 \global\let\epsfpercent=%\global\def\epsfbblit{%BoundingBox}}%
%
%   So we're ready to check for `%BoundingBox:' and to grab the
%   values if they are found.
%
\long\def\epsfaux#1#2:#3\\{\ifx#1\epsfpercent
   \def\testit{#2}\ifx\testit\epsfbblit
      \epsfgrab #3 . . . \\%
      \epsffileokfalse
      \global\epsfbbfoundtrue
%-% Don't stop if line does not start with %.  May be (at end) or binary stuff
%  \fi\else\ifx#1\par\else\epsffileokfalse\fi\fi}%
   \fi\else\ifx#1\par\else\fi\fi}%
%
%   Here we grab the values and stuff them in the appropriate definitions.
%
\def\epsfempty{}%
\def\epsfgrab #1 #2 #3 #4 #5\\{%
\global\def\epsfllx{#1}\ifx\epsfllx\epsfempty
      \epsfgrab #2 #3 #4 #5 .\\\else
   \global\def\epsflly{#2}%
   \global\def\epsfurx{#3}\global\def\epsfury{#4}\fi}%
%
%   We default the epsfsize macro.
%
\def\epsfsize#1#2{\epsfxsize}
%
%   Finally, another definition for compatibility with older macros.
%
\let\epsffile=\epsfbox

\catcode`\`=\quoteleftcode		% restore previous catcode
